B-fields In STar-forming Region Observations (BISTRO): Population-Level Universality and Environmental Structuring of 450/850 $\mu$m Polarization Signatures

We observed 69 molecular cloud regions at 450 and 850 $\mu$m with the POL-2 polarimeter on the James Clerk Maxwell Telescope and matched the maps to a common $12.6''$ beam. Polarization fractions are typically lower at 450 $\mu$m. The median of 30 measured ratios is $P_{450}/P_{850} = 0.69 \pm 0.02_{\rm sys} \pm 0.03_{\rm stat}$. Across 35 regions with reliable spectral indices of total ($\alpha$) and polarized ($\gamma$) intensity, the medians over sources are $\langle\alpha\rangle = 3.33$ and $\langle\gamma\rangle = 2.85$-$3.04$. The median $\gamma - \alpha$ is $-0.57$ to $-0.45$, with $\gamma < \alpha$ in 24-27 regions. These ranges span the two extreme placements of $3\sigma$ limits for polarized intensity below the noise floor. The position angles at the two wavelengths agree within $10^\circ$ in 10 of 13 regional medians, disfavoring a geometric origin that would rotate the angles. The medians of $\gamma-\alpha$ in 9 low-mass, 19 high-mass and 7 Central Molecular Zone (CMZ) regions are not ordered low-mass $<$ high-mass $<$ CMZ (Jonckheere-Terpstra $p = 0.43$-$0.70$). A difference among classes is not robustly detected. The Kruskal-Wallis $p = 0.056$-$0.078$ becomes $p = 0.026$-$0.041$ when the Rosette Molecular Cloud alone is excluded, although the high-mass class has the lowest median in every treatment. The classes follow a distance sequence (the beam spans 0.008-0.51 pc), coupling environment and physical scale. Within clouds, the 450 $\mu$m polarization fraction decreases with Herschel column density in all 7 fields with sufficient dynamic range. Coefficients from pooled pixels mix trends within clouds, differences between clouds, and the influence of OMC 1. They therefore do not define a single law for individual pixels. The wavelength dependence across sources provides a benchmark for grain alignment. We cannot order it by environment and do not propose a unique mechanism.

==> xref_frozen_S2_pasj.tex <==
\makeatletter
\newlabel{S1-app:F1_uncorrected}{{5}{38}{}{section.\theH@article .5}{}}
\newlabel{S1-app:Tmixing}{{3}{35}{}{section.\theH@article .3}{}}
\newlabel{S1-fig:IratioRp}{{4}{18}{}{figure.\theH@article .4}{}}
\newlabel{S1-fig:PA450vsPA850}{{2}{15}{}{figure.\theH@article .2}{}}
\newlabel{S1-fig:Pratio_OphA_method3}{{3}{16}{}{figure.\theH@article .3}{}}
\newlabel{S1-fig:PvsS}{{7}{23}{}{figure.\theH@article .7}{}}
\newlabel{S1-sec:obs}{{2}{9}{}{section.\theH@article .2}{}}
\newlabel{S1-sec:results}{{3}{13}{}{section.\theH@article .3}{}}
\newlabel{S1-ss:Discussion_GammaAlpha}{{4.2}{25}{}{subsection.\theH@article .2}{}}
\newlabel{S1-ss:Discussion_theory}{{4.3}{26}{}{subsection.\theH@article .3}{}}
\newlabel{S1-ss:Iratio}{{3.3}{17}{}{subsection.\theH@article .3}{}}
\newlabel{S1-ss:P_ratio}{{3.2}{14}{}{subsection.\theH@article .2}{}}
\newlabel{S1-ss:S_dispersion}{{3.5}{20}{}{subsection.\theH@article .5}{}}
\newlabel{S1-ss:SpIdx}{{3.4}{17}{}{subsection.\theH@article .4}{}}
\newlabel{S1-ss:bfield_consistency}{{3.1}{13}{}{subsection.\theH@article .1}{}}
\newlabel{S1-ss:samples}{{2.4}{12}{}{subsection.\theH@article .4}{}}
\newlabel{S1-tbl:S1_F1F3_master}{{2}{8}{}{table.\theH@article .2}{}}
\newlabel{S1-tbl:S1_dependency}{{3}{10}{}{table.\theH@article .3}{}}
\newlabel{T-app:QU_diagnostics}{{2}{61}{}{section.\theH@article .2}{}}
\newlabel{T-app:ricean}{{1}{59}{}{section.\theH@article .1}{}}
\newlabel{T-eq:precision_floors}{{57}{53}{}{equation.\theH@article .57}{}}
\newlabel{T-fig:SpIdx_BiasCheck_OphA}{{14}{32}{}{figure.\theH@article .14}{}}
\newlabel{T-sec:obs}{{2}{6}{}{section.\theH@article .2}{}}
\newlabel{T-sec:precisionfloor}{{4.2}{53}{}{subsection.\theH@article .2}{}}
\newlabel{T-sec:uncertainty}{{4.1}{50}{}{subsection.\theH@article .1}{}}
\newlabel{T-ss:beamval}{{3.5}{45}{}{subsection.\theH@article .5}{}}
\newlabel{T-ss:flux}{{3.1}{7}{}{subsection.\theH@article .1}{}}
\newlabel{T-ss:noiseI}{{3.2}{11}{}{subsection.\theH@article .2}{}}
\newlabel{T-ss:noisemodel}{{3.3}{24}{}{subsection.\theH@article .3}{}}
\newlabel{T-ss:obs_reduction}{{2.3}{7}{}{subsection.\theH@article .3}{}}
\newlabel{T-ss:offset}{{3.4}{32}{}{subsection.\theH@article .4}{}}
\newlabel{T-ss:spidx_snrbias}{{3.3.7}{31}{}{subsubsection.\theH@article .7}{}}
\newlabel{T-ss:spidx_snrbias_sens}{{3.3.9}{31}{}{subsubsection.\theH@article .9}{}}
\newlabel{T-tbl:T_sample_inventory}{{2}{6}{}{table.\theH@article .2}{}}
\newlabel{T-tbl:systematics}{{7}{52}{}{table.\theH@article .7}{}}
\makeatother

